ScanGAN360: A Generative Model of Realistic Scanpaths for 360$^{\circ}$ Images

Understanding and modeling the dynamics of human gaze behavior in 360$^\circ$ environments is a key challenge in computer vision and virtual reality. Generative adversarial approaches could alleviate this challenge by generating a large number of possible scanpaths for unseen images. Existing methods for scanpath generation, however, do not adequately predict realistic scanpaths for 360$^\circ$ images. We present ScanGAN360, a new generative adversarial approach to address this challenging problem. Our network generator is tailored to the specifics of 360$^\circ$ images representing immersive environments. Specifically, we accomplish this by leveraging the use of a spherical adaptation of dynamic-time warping as a loss function and proposing a novel parameterization of 360$^\circ$ scanpaths. The quality of our scanpaths outperforms competing approaches by a large margin and is almost on par with the human baseline. ScanGAN360 thus allows fast simulation of large numbers of virtual observers, whose behavior mimics real users, enabling a better understanding of gaze behavior and novel applications in virtual scene design.

==> 5_Behavior.tex <==
\section{Behavioral evaluation}
\label{sec:behavior}

\belen{This is now copy-paste of the main paper section we submitted to SIGG. The next two secs of the supplementary need to be merged into this section (and perhaps the section rewritten a bit once the corresponding one in the main paper is final).}


\begin{figure*}[t!]
	\centering
	\includegraphics[width=\linewidth]{figures/sal_roc_time.jpg}
	\caption{Behavioral evaluation. Left: Exploration time computed as the average time until a certain longitudinal offset from the starting point is reached, for both real captured data (left) and scanpaths generated by our model (center left). Speed and exploration time of our scanpaths are on par with that of real users. Center right: ROC curve of our generated scanpaths as a measure of inter-observer congruency, for each individual test scene (gray), and averaged across scenes (magenta). The faster it converges to the maximum rate, the higher the congruency. Right: Aggregate maps for two different scenes, computed as heatmaps from 1,000 generated scanpaths. Our model is able to produce aggregate maps that focus on relevant areas of the scenes and exhibit the previously reported equator bias.}
	\label{fig:exploTime}
\end{figure*}

The analysis presented in the previous section evaluates whether the scanpaths generated with our model are close to the ground truth ones, and how they compare with those of related works. This is done with a number of metrics from the literature that analyze different characteristics of the scanpaths: shape, distances between points, cross-recurrence, etc. In this section, we perform a higher-level analysis, assessing whether the behavioral characteristics of our generated scanpaths match those which have been studied and reported from actual users watching 360$^\circ$ images.


\paragraph{Temporal and spatial coherence} 
Our generated scanpaths have a degree of stochasticity, to be able to model the behavior of different users. However, human gaze behavior follows specific patterns, and each gaze point is conditioned not only on the features in the scene but also by the previous history of gaze points of the user. If two users start watching a scene in the same region, a certain degree of coherence between their scanpaths is expected, that may diverge more as more time passes. We therefore analyze the temporal coherence of our generated scanpaths that start in the same region. Specifically, we do this by generating a set of random scanpaths for each of the scenes in our test dataset, and separate them according to the longitudinal region where the scanpath begins (\eg, $[0^\circ, 40^\circ), [40^\circ,80^\circ)$, etc.). Then, we estimate the probability density of the generated scanpaths from each starting region using kernel density estimation (KDE) for each timestamp. \iccvNew{This is NO LONGER shown in Figure~\ref{fig:kde} for two different starting regions of the $chess$ scene, at four different timestamps, and computed over 1000 generated scanpaths}. During the first seconds (first column), gaze points tend to stay in a smaller area, and closer to the starting region; as time progresses, they exhibit a more exploratory behavior with higher divergence, and eventually may reach a convergence close to regions of interest. We can also see how the behavior can differ depending on the starting region: at 10 seconds (second column), in the top row most of the attention is focused on the black pieces, while in the bottom row the attention is split between two large regions. The supplementary video and Section S8 in the supplementary material contain more results, including different scenes and the whole set of starting regions. 


\paragraph{Exploration time} Previous work has studied viewing behavior of users when watching a 360$^\circ$ scene, including the speed with which users explore the scene~\cite{sitzmann2018saliency}. Sitzmann et al.~\cite{sitzmann2018saliency} measure the \emph{exploration time} as the average time that users took to move their eyes to a certain longitude relative to their starting point, and measure how long it takes for users to fully explore the scene. Figure~\ref{fig:exploTime} (left) shows this exploration time, measured by Sitzmann et al. from captured data, for the three scenes from their dataset included in our test set (\emph{room}, \emph{chess}, and \emph{robots}). We wish to analyze whether our generated scanpaths mimic this behavior and exploration speed, and plot the exploration time of our generated scanpaths (Figure~\ref{fig:exploTime}, center left) for the same scenes and number of scanpaths. We can see how the speed and exploration time are very similar between real and generated data. Individual results per scene can be found in Section S9 in the supplementary material.



\paragraph{Fixation bias} Following studies that have reported a strong bias of human fixations towards the center of regular images~\cite{judd2009learning}, works have analyzed biases when viewing 360$^\circ$ content. The existence of a strong Laplacian-like equator bias has been shown~\cite{sitzmann2018saliency}: the majority of fixations fall around the equator, in detriment of the poles. This behavior has been associated with the placement of relevant content at the equator in most of the 360º layouts used in virtual environments. We have evaluated whether the distribution of scanpaths generated by our model also presents this bias. This is to be expected, since the data our model is trained with exhibits it, but is yet another indicator that we have succeeded in learning the ground truth distribution. We test this by generating, for each scene, 1000 different scanpaths with our model, and aggregating them over time to produce a \emph{pseudo-}saliency map, which we term \emph{aggregate map}. Figure~\ref{fig:exploTime} (right) 
shows this for two scenes in our test set: We can see how this equator bias is indeed present in our generated scanpaths.

\paragraph{Inter-observer congruency} It is common in the literature analyzing users' gaze behavior to measure inter-observer congruency, often by means of a receiver operating characteristic (ROC) curve. We compute the congruency of our ``generated observers'' through this ROC curve for the three scenes in our test set from the Sitzmann et al. dataset (Figure~\ref{fig:exploTime}, center right). The curve calculates the ability of the $i^{th}$ scanpath to predict the aggregate map of the corresponding scene.  
Each point in the curve is computed by generating a map containing the top $n\%$ most salient regions of the aggregate map (computed without the $i^{th}$ scanpath), and calculating the percentage of gaze points of the $i^{th}$ scanpath that fall into that map. Our ROC curve indicates a strong agreement between our scanpaths, with around $75\%$ of all gaze points falling within $25\%$ of the most salient regions. These values are comparable to those measured in previous studies with captured gaze data~\cite{sitzmann2018saliency,lemeur2013}.


\endinput

The metrics presented in the previous section allow to analyze and validate whether the produced scanpaths can fit in a real scanpath distribution, giving their different characteristics about shape, distances, or cross-recurrence, or the spatial and temporal similarities between them. However, human viewing behavior in VR is more complex: It presents some biases~\citep{sitzmann2018saliency}, and there are some aspects that define human visual exploration. In this section, we have analyzed different aspects that characterize human viewing behavior, to validate that our produced scanpaths can indeed mimic real human patterns.


\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/roc_time.jpg}
	\caption{Exploration time computed as the average time until certain longitudinal offsets from the starting point are reached, for both real data and our method. On average, the scanpaths generated with our model explore the whole scene in approximately 16 seconds, which is almost on pair with previous studies~\cite{sitzmann2018saliency}. \belen{Both are same nr of ppl now.}}
	\label{fig:time_roc}
\end{figure}


\paragraph{Starting point and exploratory behavior} We firstly explored whether our generated scanpaths are actually temporally coherent: Although the gaze points that our model generates are correctly distributed over a given scene, we also analyzed whether their exploratory patterns are meaningful. When humans explore virtual scenes, they tend to firstly explore areas closer to the starting point, to then explore further regions of the scene. To analyze if our model also follows this trend, we generate a set of random scanpaths for each of the scenes of our test dataset. We then separate the scanpaths depending on their longitudinal starting range, and compute the kernel density estimation (KDE) for different timestamps for each of them (see Figure~\ref{fig:kde}). During the first seconds, gaze points tend to stay in a closer area near the beginning, whilst they get a more exploratory behavior over time, until reaching a convergence close to regions of interest. Please refer to Section~\dani{SXX} in the supplementary material for the complete set of KDE results over the three evaluation images.


\begin{figure*}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/kdes_2.jpg}
	\caption{In order to verify whether our scanpaths are meaningful and realistic, we analyze their exploratory behavior over time, depending on the starting point. For this figure, we take a set of 1000 scanpath starting at two different longitudinal ranges (depicted in red in the first image of each row, including ranges from 0$^{\circ}$ to 20$^{\circ}$ (\ie, the left-most part of the image), and from 160$^{\circ}$ to 180$^{\circ}$ (\ie, the center of the image)), and for each of them, we show the kernel density estimation (KDE) of gaze points at four different timestamps $t = \{2, 10, 20, 30\}$ seconds. Our scanpaths' behavior is tied to the starting point, but always respect a similar pattern: They have a more exploratory behavior in early stages, whereas they tend to converge over time.}
	\label{fig:kde}
\end{figure*}




\paragraph{Time to explore the scene} As aforementioned, viewing patterns depend on the starting point of the scene, since users are more prone to explore areas closer to the starting one in the first seconds, whilst their behavior become more sparse over time, up to a point where the whole scene is completely explored, which has been reported to occur after around 19 seconds~\citep{sitzmann2018saliency}. Following a similar fashion, we also analyze the speed of exploration of our scanpaths (\ie, the time it takes our scanpaths to reach certain longitudinal positions based on their starting points). On average, the scanpath generated with our model fully explore a 360º scene in approximately 16 seconds, (see Figure~\ref{fig:time_roc}), which is similar to those previous works, proving our scanpaths to follow a similar fashion as humans regarding exploration speed and time. Please refer to Section~\dani{SXX} in the supplementary material for both the ground truth and the individual results of the three evaluation scenes.


\paragraph{Scanpath convergence in saliency} Saliency is computed by aggregating multiple users' fixations over time, so that the areas that have drawn the more attention from the users are considered more salient. Saliency is commonly depicted as a heatmap with values $s \in [0,1]$, with higher values indicating a higher saliency. To compute a baseline saliency map for a given scene, multiple users are presented that specific scene, and their gaze points (or sometimes their head orientation, as proven to be a good proxy~\cite{sitzmann2018saliency}) are recorded over time, to then be aggregated into a final saliency map. Since our model is able to potentially mimic human behavior, we prove that a big, variate enough set of scanpaths generated with our model can be used to compute saliency maps (see Figure~\ref{fig:saliency}).


\begin{figure*}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/saliency.jpg}
	\caption{For two scenes from our test set separated from Sitzmann et al~\citep{sitzmann2018saliency}, and two scenes from Rai et al.'s dataset~\cite{rai2017dataset}, we show the saliency map computed by aggregating 100 scanpaths randomly generated with our model over each of them. Our method is able to generate realistic scanpaths, and the saliency map computed from them actually accounts for the more relevant parts of the scene. }
	\label{fig:saliency}
\end{figure*}



\paragraph{Human fixation bias} As many studies reported a strong bias for human fixations towards the center of regular images~\cite{judd2009learning}, some works were also devoted to analyze if similar behaviors hold in VR, reporting the existence of a strong Laplacian-like equator bias~\cite{sitzmann2018saliency}, where most of human fixations fall in the equator. This behavior has been associated to a clear horizon line in most of the 360º layouts used in virtual environments. We have evaluated whether the distribution of our model also presents this bias. For each of the scenes of our evaluation dataset, we generated 1000 different scanpaths and computed their average saliency map, which also resulted biased towards the equator (see two examples in Figure~\ref{fig:saliency}), which is also shared with human behavior in virtual environments. We hypothesize that our model is biased due to the inherent bias of both the location of features in our dataset and the ground truth scanpaths used in training. However, as already reported~\cite{sitzmann2018saliency}, most of 360º content presents that clear horizon line, with most of the salient, relevant elements close to it, and therefore our model bias is reasonable. Further analysis on 360$^{\circ}$ scenes where there is no clear horizon line remains as a future avenue.


\paragraph{Congruence between scanpaths} Although there is variance between different users' exploratory behavior, and even in how a specific user behaves when exploring different scenes, humans tend to direct their attention to the most salient parts of the scene. We also analyze whether our model is able to generate scanpaths that yield a similar agreement. We thus compute a \textit{receiver operating characteristic} curve (ROC), which calculates the ability of the $i^{th}$ generated scanpath to predict a ground truth saliency map computed by means of aggregating the gaze points of the rest of the scanpaths. Each point in the curve is hence computed calculating the percentage of gaze points of the $i^{th}$ scanpath that fall into the heatmap containing the $n\%$ most salient regions aggregating the rest of the scanpaths' points. 
Our results indicate a strong agreement between our scanpaths, with a $65\%$ of all gaze points falling within the $20\%$ most salient regions of the scene.



==> 8_Conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

\gordon{this section is currently a summary of what we did, which is very different from a conclusion. you can briefly summarize what you did in the beginning of the discussion section, but not here. In the conclusions, you should briefly say how everything we learned in this paper will have a big impact on the field of computer graphics and interactive techniques.}

\dani{Revisit when everything is done again}

To our knowledge, we have presented the first completely spherical-aware generative adversarial framework to generate plausible, realistic human scanpaths for 360$^{\circ}$ content, with a time-window much longer than previous state-of-the-art works, and without resorting to any static importance notion, such as saliency. We have also presented the not only the first approach to using a time series DTW-based loss function to enhance our model performance, but also a novel, spherical-aware adaptation of it, allowing our model to inherently learning all the spatiotemporal coherence of the scanpaths at once. We have qualitatively and quantitatively evaluated our model against previous approaches, proving our model to be the most precise and accurate in terms of a wide, variate enough set of metrics that are specifically designed to evaluate and compare different attributes of scanpaths. Moreover, our model generates scanpaths that actually mimic human behavior, maintaining different exploratory patterns that commonly show up in real humans when exploring this type of content. We have also demonstrated that our generated scanpaths are robust, and can be useful to address several problems: \dani{visual guiding, blah blah},  \dani{foveated rendering, blah blah}, exploring 360$^{\circ}$ content in traditional, 2D displays,  or \dani{deisgning virtual avatars, blah blah}. We believe our hope helps further understand human viewing behavior, and hope future work will leverage and improve our framework.
